Generalized Reduced-Rank Regression with Homogeneity Pursuit

Homogeneity, low rank, and sparsity are three widely adopted assumptions in multi-response regression models to address the curse of dimensionality and improve estimation accuracy. However, there is limited literature that examines these assumptions within a unified framework. In this paper, we investigate the homogeneity, low rank, and sparsity assumptions under the generalized linear model with high-dimensional responses and covariates, encompassing a wide range of practical applications. Our work establishes a comprehensive benchmark for comparing the effects of these three assumptions and introduces a regularized maximum likelihood estimation method to fit the corresponding models. Under mild conditions,we prove the statistical consistency of our estimator. Theoretical results provide insights into the role of homogeneity and offer a quantitative analysis of scenarios where homogeneity improves estimation accuracy. The proposed method's effectiveness is demonstrated through numerical simulations and an empirical analysis of tree species data from Barro Colorado Island.

==> proof.tex <==
\appendix

\input{v5.tex}




==> proofs/lemmas.tex <==
\section{Supplementary Proofs for Theoretical Results}
\subsection{Proofs of Proposition \ref{prop:4}}

Recall the negative log-likelihood is defined as
\begin{align*}
	\ell(\bA,\bB) = \sum_{i=1}^n b(\bA\trans\z_i + \bB\trans\x_i) - \sum_{i=1}^n \sum_{j=1}^m y_{ij}(\balpha_j\trans\z_i + \bbeta_j\trans\x_i),
\end{align*}
where $\bA=[\balpha_1,\dots,\balpha_m]$ and $\bB = [\bbeta_1,\dots,\bbeta_m]$. For the sake of clarity, we let $\btheta_i\in \mbR^m$ be $\bA\trans\z_i + \bB\trans\x_i$ then the quadratic approximation of $\ell(\bA,\bB)$ is
\begin{align*}
	\ell(\bA,\bB)
	 & \approx \frac{1}{2} \sum_{i=1}^n \inner{\nabla^2 b(\btheta_i^t)(\btheta - \btheta_i^t), \btheta_i - \btheta_i^t} + \sum_{i=1}^n \inner{\nabla b(\btheta_i^t) - \y_i, \btheta_i - \btheta_i^t}
	 + \sum_{i=1}^n \inner{\nabla b(\btheta_i^t), \btheta_i^t} + \sum_{i=1}^n b(\btheta_i^t),
\end{align*}
where $\btheta_i^t = (\bA^t)\trans\z_i + (\bB^t)\trans \x_i$. Then we consider the majorizing function of the negative log-likelihood by two cases.

\noindent\underline{(1) Multinomial logistic model.} Under the multinomial logistic model, there is
\begin{align*}
	\nabla b(\btheta_i^t) = \p_i^t \in \mbR^m
	, \quad
	\nabla^2 b(\btheta_i^t) = \diag{\p_i^t} - \p_i^t(\p_i^t)\trans \in \mbR^{m\times m},
\end{align*}
where the $j$-th component ($p_{ij}^t$) of $\p_i^t$ is $\exp(\theta_{ij}^t) / [1 + \sum_{j=1}^m \exp(\theta_{ij}^t)]$ with $j = 1,\dots,m$. By Lemma 3.3 in \citet{simon2013blockwise}, let $w_t = \max_{i,j} 2 p_{ij}^t (1 - p_{ij}^t)$ then there is $\nabla^2 b(\btheta_i) \preceq w_t\bI$ for all $i=1,\dots,n$. Together with the convexity of $\ell(\bA,\bB)$, we have
\begin{align*}
	\ell(\bA, \bB)
	 & \leq
	\frac{w_t}{2} \sum_{i=1}^n \norm{\frac{\nabla b(\btheta_i^t) - \y_i}{w_t} + \btheta_i - \btheta_i^t}_2^2
	\underbrace{- \frac{w_t}{2} \sum_{i=1}^n \norm{\frac{\nabla b(\btheta_i^t) - \y_i}{w_t}}_2^2 + \sum_{i=1}^n \inner{\nabla b(\btheta_i^t), \btheta_i^t} + \sum_{i=1}^n b(\btheta_i^t)}_{\text{constant:}~ C_t}.
\end{align*}
Therefore, we can consider the surrogate loss function as follows
\begin{align}
	\ell^S(\bA, \bB) = \frac{w_t}{2} \sum_{i=1}^n \norm{\y_i^t - \bA\trans\z_i - \bB\trans\x_i}_F^2 = \frac{w_t}{2} \norm{\bY^t - \bZ\bA - \bX\bB}_F^2, \label{prop:4:eq:1}
\end{align}
where $\y_i^t = \btheta_i^t + (\y_i - \nabla b(\btheta_i^t)) / w_t$, $w_t = \max_{i,j} 2 p_{ij}^t (1 - p_{ij}^t)$ and we omit the constant $C_t$. Moreover, denote the $j$-th diagonal component of the Hessian $\nabla^2 b(\btheta_i)$ by $\nabla^2 b_j(\theta_{ij})$ then there is $w_t = \max_{i,j} 2 \nabla^2 b_j(\theta_{ij}^t)$.

\noindent\underline{(2) Generalized linear model.} Note that $\nabla^2 b(\btheta_i^t)$ is a $m\times m$ diagonal matrix and let $\nabla^2 b_j(\theta_{ij}^t)$ be its $j$-th diagonal component. There is $\nabla^2 b(\btheta_i^t) \preceq w_t \bI$ with $w_t = \max_{i,j} \nabla^2 b_j(\theta_{ij}^t)$. Thus following the same argument, we can consider the surrogate loss function that has the same formulation as \eqref{prop:4:eq:1} but $w_t = \max_{i,j} \nabla^2 b_j(\theta_{ij}^t)$.

\subsection{Proofs of Proposition \ref{prop:3}}

Let $\wt \bL$ be the unnormalized Laplacian matrix then by direct calculations, we have
\begin{align*}
	\trace{\bB\wt\bL\bB\trans}
	 & = \trace{\bB\bD\bB\trans} - \trace{\bB\bA\bB\trans}
	= \sum_{i=1}^m d_i \norm{\bbeta_i}_2^2 - \sum_{k=1}^K \sum_{i,j\in G_k} \bbeta_i\trans\bbeta_j\\
	&= \sum_{k=1}^K \sum_{i,j \in G_k} \norm{\bbeta_i - \bbeta_j}_2^2,
\end{align*}
where $\bbeta_i\in \mbR^p$ is the $i$-th column of $\bB$, $\bA$ and $\bD$ are the adjacency matrix and degree matrix, respectively. Without loss of generality, we conside the $k$-th cluster $G_k$ and there is
\begin{align*}
	\sum_{i,j\in G_k} \norm{\bbeta_i - \bbeta_j}_2^2
	 & = \sum_{i,j\in G_k} (\norm{\bbeta_i}_2^2 + \norm{\bbeta_j}_2^2 - 2\bbeta_i\trans\bbeta_j)
	= 2\abs{G_k}\sum_{i\in G_k} \norm{\bbeta_i}_2^2 - 2\sum_{i,j\in G_k} \bbeta_i\trans\bbeta_j
	\\
	 & = 2\abs{G_k}\sum_{i\in G_k} \norm{\bbeta_i}_2^2 - 2\abs{G_k}^2 \norm{\m_k}_2^2
	= 2\abs{G_k} \sum_{i\in G_k} \norm{\bbeta_i - \m_k}_2^2,
\end{align*}
with $\m_k = \abs{G_k}^{-1} \sum_{i\in G_k} \bbeta_i$. Recall the definition that $\bW$ is the $m\times m$ diagonal matrix, whose $j$-th diagonal entry is equal to $1/\abs{G_k}$ and the normalized Laplacian matrix $\bL = \bW^{-1/2}\wt\bL\bW^{-1/2}$. Therefore, we have
\begin{align*}
	\trace{\bB\bL\bB\trans} = \trace{\bB\bW^{-1/2}\wt\bL\bW^{-1/2}\bB\trans} = 2\sum_{k=1}^K \sum_{j\in G_k} \norm{\bbeta_j - \m_k}_2^2,
\end{align*}
which finishes the proof.

\subsection{Proofs of Theorem \ref{thm:2}}

We just need to demonstrate that $L_t(\bA^t, \bU^t, \bV^t, \mbG^t) \geq L_t(\bA^{t+1}, \bU^{t+1}, \bV^{t+1}, \mbG^{t+1})$, where $L(\bA, \bU, \bV, \mbG)$ is the majorizing objective function defined in \eqref{opt:4}.

\noindent\underline{(1) Convergence of the update for $\bU$.} The objective function for the update of $\bU$ is
\begin{align*}
	L_t(\bU)
	 & = \frac{w_t}{2} \norm{\bY^t - \bZ\bA^t - \bX\bU(\bV^t)\trans}_F^2 + \frac{\lambda}{2} \trace{\bU(\bV^t)\trans\bL^t\bV^t\bU\trans}
	\\
	 & = \frac{w_t}{2} \trace{\bU\trans\bX\trans\bX\bU} + \frac{\lambda}{2}\trace{\bU(\bV^t)\trans\bL^t\bV^t\bU\trans} - w_t\times \trace{(\bV^t)\trans(\wt{\bY}^t)\trans\bX\bU} + \text{const},
\end{align*}
where we denote $\wt{\bY}^t = \bY^t - \bZ\bA^t$ by the centered response matrix for convenience. For two arbitrary $\bU_1$ and $\bU_2$, there is
\begin{align*}
	 & L_t(\bU_2) - L_t(\bU_1)
	= \frac{w_t}{2} \trace{(\bU_2 - \bU_1)\trans\bX\trans\bX(\bU_2 - \bU_1)}
	\\
	 & \quad
	+ \frac{\lambda}{2}\trace{(\bU_2-\bU_1)(\bV^t)\trans\bL^t\bV^t(\bU_2-\bU_1)\trans}
	+ \inner{\nabla L(\bU_1), \bU_2 - \bU_1}.
\end{align*}
If the $\bU_1,\bU_2$ satisfies $\norm{\bU_l}_{2,0}\leq s$ with $l=1,2$, together with Condition \ref{cond:1}, we know that with some constant $C>0$, there is
\begin{align*}
	\norm{\bX(\bU_2 - \bU_1)}_F^2 \geq C n\kappa \norm{\bU_2 - \bU_1}_F^2.
\end{align*}
On the other hand, we have $\norm{\bX(\bU_2 - \bU_1)}_F^2 \leq \norm{\bX}_{2s,\op}^2 \norm{\bU_2 - \bU_1}_F^2$. Since the eigenvalues of $\bL$ is bounded between $0$ and $2$, we can obtain that
\begin{align*}
	Cn\kappa \norm{\bU_2 - \bU_1}_F^2
	\leq
	L_t(\bU_2) - L_t(\bU_1) - \inner{\nabla L_t(\bU_1), \bU_2 - \bU_1}
	\leq
	\left(\norm{\bX}_{\op,2s}^2 + \lambda\right) \norm{\bU_2 - \bU_1}_F^2.
\end{align*}
Therefore, the objective function satisfies the restricted strong convexity and strong smooth conditions. Following Theorem 1 of \citet{jain2014iterative}, we know that the hard-threshold gradient descent decreases the objective function that is $L_t(\bU^{t+1}) \leq L_t(\bU^t)$ with the step size $\eta = O\left(n\kappa/(\norm{\bX}_{2s,\op} + \lambda)\right)$.

\smallskip

\noindent\underline{(2) Convergence of the update for $\bV$.} By the definition of $\m_j^{t+1}$, it holds that
\[
	\sum_{k = 1}^K \sum_{j\in G_k^t} \norm{\bU^{t+1}(\v_j^{t+1} - \m_k^{t+1})}_2^2 \le \sum_{k = 1}^K \sum_{j\in G_k^t} \norm{\bU^{t+1}(\v_j^{t+1} - \m_k^t)}_2^2,
\]
which suggests that
\begin{align*}
	 & \frac{w_t}{2} \norm{\bY^t - \bZ\bA^t - \bX\bU^{t+1}(\bV^{t+1})\trans}_F^2 + \frac{\lambda}{2}\trace{\bU^{t+1}(\bV^{t+1})\trans\bL^t\bV^{t+1}(\bU^{t+1})\trans}
	\\
	 & \quad = \frac{w_t}{2} \norm{\bY^t - \bZ\bA^t - \bX\bU^{t+1}(\bV^{t+1})\trans}_F^2 + \lambda \sum_{k=1}^K \sum_{j\in G_k^t} \norm{\bU^{t+1}(\v_j^{t+1} - \m_k^{t+1})}_F^2
	\\
	 & \quad \leq \frac{w_t}{2} \norm{\bY^t - \bZ\bA^t - \bX\bU^{t+1}(\bV^{t+1})\trans}_F^2 + \lambda \sum_{k=1}^K \sum_{j\in G_k^t} \norm{\bU^{t+1}(\v_j^{t+1} - \m_k^{t})}_F^2
	\\
	 & \quad \leq \frac{w_t}{2} \norm{\bY^t - \bZ\bA^t - \bX\bU^{t+1}(\bV^{t})\trans}_F^2 + \lambda \sum_{k=1}^K \sum_{j\in G_k^t} \norm{\bU^{t+1}(\v_j^{t} - \m_k^{t})}_F^2
	\\
	 & \quad = \frac{w_t}{2} \norm{\bY^t - \bZ\bA^t - \bX\bU^{t+1}(\bV^{t})\trans}_F^2 + \frac{\lambda}{2}\trace{\bU^{t+1}(\bV^{t})\trans\bL^t\bV^{t}(\bU^{t+1})\trans},
\end{align*}
where the second last inequality follows from the fact that $\bV^{t+1}$ minimizes~\eqref{V1} with $\m_k=\m_k^{t}={\abs{G_k^t}}^{-1} \sum_{j\in G_k^t}\v_j^t$. Therefore, the update algorithm of $\bV$ ensures the value of objective function is descending.

\smallskip

\noindent\underline{(3) Convergence of the update for the intercept and clusters.} It is obvious that the update of $\bA$ decreases the loss function by its definition. As for the update of $\{G_k\}_{k=1}^K$, it is the standard $K$-means clustering, which ensures the fusion penalty is descending. Therefore, the update of clusters also decreases the objective function since the the loss function term is fixed. Finally, with the descent of surrogate function, the majorize-minimization framework guarantees the descent of the original objective function \citep{lange2016mm}.
% Following the above analysis, we have that $L_t(\bA^t, \bU^t, \bV^t, \mbG^t) \geq L_t(\bA^{t+1}, \bU^{t+1}, \bV^{t+1}, \mbG^{t+1})$. Since the surrogate loss function $\ell^S(\bA,\bU,\bV) + C_t$ majorizes the negative log-likelihood by Proposition \ref{prop:4}, we have
% \begin{align*}
% 	 & \mcL(\bA^t,\bU^t,\bV^t,\mbG^t) \geq
% 	L_t(\bA^{t},\bU^{t},\bV^{t},\mbG^{t}) + C_t
% 	\geq L_t(\bA^{t+1},\bU^{t+1},\bV^{t+1},\mbG^{t+1}) + C_t
% 	\\
% 	 & \quad \geq \mcL(\bA^{t+1},\bU^{t+1},\bV^{t+1},\mbG^{t+1}),
% \end{align*}
% which demonstrates the algorithm decrease the objective function.


\section{Auxiliary Lemmas}

\begin{lemma}\label{lem:2}
	Under Condition \ref{cond:4}, for any $(p+q)\times m$ matrix $\bQ$ such that $\norm{\bQ}_{2,0}\le s$, it holds for any $\gamma>0$ that
	\begin{align}
 \label{eq:lem:2}
\mbP\left(\left|\inner{\bQ,\nabla \ell(\bA,\bB) - \mbE\left[\nabla \ell(\bA,\bB)\right]}\right| > \gamma\right)\le 2 \exp\left(-\frac{\gamma^2}{\tau \norm{\wt \bX}_{s,op}^2\|\bQ\|_F^2}\right).
	\end{align} 
\end{lemma}
\begin{proof}{Proof.}
Denote $\bmu_i = \partial b / \partial \btheta_i \in \mbR^m$ with $\btheta_i = \bA\trans\z_i + \bB\trans\x_i$, then we can write the $\nabla \ell(\bA,\bB)$ as follows
\begin{align*}
	\nabla \ell(\wt\bB) = \sum_{i=1}^n \wt\x_i (\bmu_i - \y_i)\trans ,
\end{align*}
where $\wt\bB = [\bA\trans,\bB\trans]\trans$ and $\wt\x_i = (\z_i\trans,\x_i\trans)\trans$. Denote by $\bmu_i^* = \mbE(\y_i)$, which equals  the derivative of $b(\btheta_i)$ evaluated at $\btheta_i^* = \bA\strans\z_i +\bB\strans \x_i$. Therefore, the expectation of $\ell(\wt\bB)$ is 
\begin{align*}
	\mbE\left[\nabla \ell(\bA,\bB)\right] = \sum_{i=1}^n \wt\x_i (\bmu_i - \bmu_i^*)\trans,
\end{align*}
which implies that
\begin{align*}
	\nabla \ell(\bA,\bB) - \mbE\left[\nabla \ell(\bA,\bB)\right]
	= \sum_{i=1}^n \wt\x_i (\bmu_i^* - \y_i)\trans 
	= - \sum_{i=1}^n \wt\x_i \e_i\trans,
\end{align*}
with $\e_i = \y_i - \mbE(\y_i)$.  Denote by $\q_j$ the $j$-th column of matrix $\bQ$, then it holds that
\begin{align}
	\mbP\left(\left|\inner{\bQ,\nabla \ell(\bA,\bB) - \mbE\left[\nabla \ell(\bA,\bB)\right]}\right| > \gamma\right)
	&=\mbP\left(\left|\trace{\sum_{i=1}^n \bQ\trans\wt\x_i \e_i\trans}\right| > \gamma\right)\nn
	=\mbP\left(\left|\sum_{i=1}^n \e_i\trans\bQ\trans\wt\x_i \right| > \gamma\right)\nn. \label{prop:2:ineq:1}
\end{align}
Under Condition~\ref{cond:4}, it holds that for any given $i$,
\[
\mbP\left(\left| \e_i\trans\bQ\trans\wt\x_i \right| > \gamma\right)\le 2\exp\left(-\frac{\gamma^2}{\tau \|\bQ\trans\wt\x_i\|_2^2}\right),
\]
which suggests that $\e_i\trans\bQ\trans\wt\x_i/\|\bQ\trans\wt\x_i\|_2$ is a sub-Gaussian random variable with a parameter $\tau$ for all $i=1,\cdots, n$. Due to the independence between $\e_i\trans\bQ\trans\wt\x_i$'s with different $i$'s,  using the the fact that sum of independent sub-Gaussian variables is still sub-Gaussian, it holds that
\[
\begin{aligned}
    \mbP\left(\left|\sum_{i=1}^n \e_i\trans\bQ\trans\wt\x_i \right|  > \gamma\right)
	&=\mbP\left(\left|\sum_{i=1}^n\|\bQ\trans\wt\x_i\|_2 \frac{\e_i\trans\bQ\trans\wt\x_i }{\|\bQ\trans\wt\x_i\|_2}\right|  > \gamma\right)
	\le 2\exp\left(-\frac{\gamma^2}{\tau \sum_{i=1}^n\|\bQ\trans\wt\x_i\|_2^2}\right)\\
    &=2\exp\left(-\frac{\gamma^2}{ \tau \sum_{i=1}^n\wt \x_i\trans\bQ\bQ\trans\wt \x_i }\right)
    \le 2\exp\left(-\frac{\gamma^2}{\tau \trace{\bQ\trans(\sum_{i=1}^n\wt\x_i\wt\x_i\trans)\bQ}}\right)
    \\
    &\le 2\exp\left(-\frac{\gamma^2}{\tau\norm{\wt \bX}_{s,op}^2 \|\bQ\|_F^2}\right).
\end{aligned}
\]
Consequently, it holds that 
\[
\mbP\left(\left|\inner{\bQ,\nabla \ell(\bA,\bB) - \mbE\left[\nabla \ell(\bA,\bB)\right]}\right| > \gamma\right)\le 2 \exp\left(-\frac{\gamma^2}{\tau \norm{\wt \bX}_{s,op}^2\|\bQ\|_F^2}\right),
\]
which completes the proof of Lemma~\ref{lem:2}.
\end{proof}

\begin{lemma}\label{lem:3} Define $S(\bA,\bB)=\ell(\bA,\bB)-\mbE\left[\ell(\bA,\bB)\right]$. Then 
	under Condition \ref{cond:4},  it holds for any $\delta>0,\gamma>0$ that
	\begin{align}
 \label{eq:lem:3}
\begin{aligned}
     \mbE&\left(\sup_{{\rm d}(\wt \bB,\wt \bB^*)\le\delta}\left| S(\bA,\bB) -  S(\bA^*,\bB^*)\right|\right)\le c\norm{\wt \bX}_{op,2s}\min(\sqrt{\gamma},\delta)\sqrt{(s+m)r}\\
     &\hskip 0.5em+c \delta \norm{\wt \bX}_{op,2s} \left(\sqrt{s\log p+m\log K}+\sqrt{[s+\min(K^2,m)]\min(r,K)\log(m)}\right),   
\end{aligned}	\end{align} 
for some constant $c>0$.
\end{lemma}

\begin{proof}{Proof.}
Denote by $\wt\bB=[\bA\trans,\bB\trans]\trans$ as the parameter matrix. Using the first order Taylor expansion, we have that $\ell(\bA,\bB)-\ell(\bA',\bB')=\inner{\wt\bB-\wt\bB', \nabla \ell(\bA'',\bB'')}$ for some $\bA''$ and $\bB''$. Then the difference between $S(\bA,\bB)$ and $S(\bA',\bB')$ can be written as 
\begin{align*}
	S(\bA, \bB) - S(\bA', \bB') 
	= \inner{\wt{\bB} - \wt{\bB}', \nabla 
	\ell(\bA'',\bB'') - \mbE\left[\nabla \ell(\bA'', \bB'')\right]}. 
\end{align*}
By invoking Lemma~\ref{lem:2}, we have that
\begin{equation}
    \mbP\left(\left|S(\bA,\bB) - S(\bA',\bB')\right| > \gamma\right)\le 2 \exp\left(-\frac{\gamma^2}{\tau \norm{\wt \bX}_{op,2s}^2(\|\bA-\bA'\|_F^2+\|\bB-\bB'\|_F^2)}\right).
\end{equation}
Therefore, $\wt S(\wt\bB)=\frac{1}{\sqrt{\tau}\norm{\wt \bX}_{op,2s}}S(\bA,\bB)$ is a sub-Gaussian stochastic process with respect the Euclidean distance ${\rm d}(\wt B,\wt B')=\sqrt{\|\bA-\bA'\|_F^2+\|\bB-\bB'\|_F^2}$ on the parameter space $\wt\mbB_{rs\gamma}$ defined in~\eqref{psp} . Then using Corollary 2.2.8 of~\cite{wellner1996weak} (page 101), it holds that
\begin{equation}
\label{con}
    \mbE\left(\sup_{{\rm d}(\wt \bB,\wt \bB^*)\le\delta}\left|\wt S(\bA,\bB) - \wt S(\bA^*,\bB^*)\right|\right)\le C\int_0^\delta\sqrt{\log \mathcal{N}\left(\epsilon/2,\wt\mbB_{rs\gamma}(\delta),{\rm d}\right)}d\epsilon,
\end{equation}
where $C$ is a university constant and $ \mathcal{N}(\epsilon/2,\wt\mbB_{rs\gamma}(\delta),{\rm d})$ is the $\epsilon/2$-covering number of the parameter space $\wt\mbB_{rs\gamma}(\delta)$ equipped with the euclidean distance ${\rm d}(\cdot,\cdot)$.

For a given $
\delta$, we can define the parameter space as following
\begin{equation}
    \label{psp}
    \begin{aligned}
    &\wt\mbB_{rs\gamma}(\delta)=\mbA(\delta)\times \mbB_{rs\gamma}(\delta) \text{ with }
    \mbA(\delta)=\{\bA:\bA\in\mbI^m,{\rm d}(\bA,\bA^*)\le\delta\}, \text{ and } \\
    &\quad \quad \mbB_{rs\gamma}(\delta)=\{\bB:\bB\in\mbI^{p\times m},\norm{\bB}_{2,0} \leq s, ~ \rank{\bB} = r,~{\rm d}(\bB,\bB^*)\le\delta, ~ \text{and} ~ P_{km}(\bB)\le \gamma\}.
    \end{aligned}
\end{equation}
It remains to find the $\epsilon$-covering number $ \mathcal{N}(\epsilon,\wt\mbB_{rs\gamma}(\delta),{\rm d})$ of $\wt\mbB_{rs\gamma}(\delta)$, i.e., to find a set $\wt\mbB_{\epsilon}=\{\wt\bB_{\epsilon,1},\cdots,\wt\bB_{\epsilon,N}, \quad N=\mathcal{N}(\epsilon,\wt\mbB_{rs\gamma}(\delta),{\rm d})\}$ such that for any $\wt \bB\in \wt\mbB_{rs\gamma}(\delta)$, there exist a $\wt\bB_{\epsilon,l}\in\wt\mbB_{\epsilon}$ such that ${\rm d}(\wt\bB,\wt\bB_{\epsilon,l})\le\epsilon$. We construct such a set $\wt\mbB_{\epsilon}$ through following steps.
\begin{enumerate}
    \item[(a).] Define $\mbA_{\alpha,\epsilon}=\{\bA_{\alpha,1},\cdots,\bA_{\alpha,N_{
    \alpha
    }}, \quad N_{\alpha}=\mathcal{N}(\epsilon,\mbA(\delta),{\rm d})\}$ such that for any $\bA\in\mbA(\delta)$, there exists a $\bA_l\in\mbA_{\alpha,\epsilon}$ such that $\|\bA-\bA_l\|_F \le\epsilon$. It readily follows that $N_{\alpha}=\mathcal{N}(\epsilon,\mbA(\delta),{\rm d}) \le \left(\frac{c\delta}{\epsilon}\right)^{mq}$ with some positive constant $c$.
    \item[(b).] To find a covering set for $\mbB_{rs\gamma}(\delta)$, it is equivalent to find the covering set for 
    \[
\Delta\mbB_{rs\gamma}(\delta)=\left\{\bDelta: \bDelta=\bB-\bB^*,\bB\in \mbB_{rs\gamma}(\delta)\right\}.
\]
It is straightforward to see that for any $\bDelta\in\Delta\mbB_{rs\gamma}(\delta)$, it holds that $\norm{\bDelta}_{2,0}\le 2s$ and that $\rank{\bDelta}\le 2r$.
  For any $\bB\in\mbB_{rs\gamma}(\delta)$, denote by matrix $\bM_{\bB}$ as the $p\times m$ the matrix whose $j$th column is the center of the cluster to which the $j$th column of $\bB$ belongs. Then we can decompose $\bDelta=\left[\bB-\bM_{\bB}-(\bB^*-\bM_{\bB^*})\right]+(\bM_{\bB}-\bM_{\bB^*})$. As a result, we can then write
\[
\Delta\mbB_{rs\gamma}(\delta)=\mbD_{rs\gamma}(\bdelta)\oplus \mbM_{rs\gamma}(\bdelta),
\]
where 
\begin{equation*}
	\begin{aligned}
		&\mbD_{rs\gamma}(\delta)=\left\{\bD: \bD=\bB-\bM_{\bB}-(\bB^*-\bM_{\bB^*}),\bB\in \mbB_{rs\gamma}(\delta)\right\}\text{ and } \\
	&\hskip 0.5em \mbM_{rs\gamma}(\delta)=\left\{\bM: \bM=\bM_{\bB}-\bM_{\bB^*},\bB\in \mbB_{rs\gamma}(\delta)\right\}.
	\end{aligned}
\end{equation*}
\item[(c).] We first analyze the property of $\mbM_{rs\gamma}(\delta)$. Recall the definition of the $K$-means homogeneity penalty
    \[
        P_{km}(\bB)=\min_{G_1,\cdots,G_k,\bmu_1,\cdots,\bmu_K}\sum_{k=1}^K \sum_{j \in G_k} \norm{\bbeta_j - \bmu_k}_2^2,
    \]
    where $\bbeta_j$ is the $j$th column of $\bB$. Therefore, for any given partition $G_1,\cdots,G_K$, $\wh\bmu_k=\frac{1}{|G_k|}\sum_{j\in G_k} \bbeta_j$. In this case, if row-rank of matrix $\bB$ is $r$, then the row rank of cluster center matrix for $\bB$, i.e., $[\wh\bmu_1;\cdots;\wh\bmu_K]_{p\times K}\in\mbI^{p\times K}$, is at most $r$. Since there are at most $K$ distinct columns in the matrix $\bM_{\bB}$, we have that $\rank{\bM_{\bB}}\le \min(r,K)$, and $\norm{\bM_{\bB}}_{2,0}\le s$, and hence that
    \begin{equation}
        \label{eq21}
                \rank{\bM_{\bB}-\bM_{\bB^*}}\le 2\min(r,K), \quad\norm{\bM_{\bB}-\bM_{\bB^*}}_{2,0}\le 2s.
    \end{equation}

Furthermore, it is straightforward to show that
\[
\norm{\bM_{\bB}-\bM_{\bB^*}}_F\le \norm{\bM_{\bB}-\bB}_F+\norm{\bB-\bB^*}_F+\norm{\bB^*-\bM_{\bB^*}}_F\le \delta+2\sqrt{\gamma} ,
\]
since $\bB,\bB^* \in \mathbb{B}_{rs\gamma}(\delta)$. 
   

In addition, there are at most $\min(K^2,m)$ distinct columns in any matrix $\bM_{\bB}-\bM_{\bB^*}$. In view of this, we can construct a space that contains all distinct columns of $\bM_{\bB}-\bM_{\bB^*}$ (after removing non-zero rows):
    \[
\mbC=\{\bC\in\mbI^{2s\times \min(K^2,m)}: \rank{\bC}\le 2\min(r,K),\norm{\mbC}_F\le \delta+2\sqrt{\gamma}\}.
    \]
Then there exists a set $\mbC_{\epsilon}=\{\bC_{\epsilon,1},\cdots,\bC_{\epsilon,N_C}\in\bC,N_C=\mathcal{N}(\frac{\epsilon}{\sqrt{m}},\mbC,\rm d)\}$ such that for any $\bC\in\mbC$, there exists a $\bC_{\epsilon,l}$ such that ${\rm d}(\bC,\bC_{\epsilon,l})\le \epsilon/\sqrt{m}$. Using the same arguments in the proof of Lemma 4 and Lemma 5 in~\cite{she2017selective},  we can show that 
\begin{align*}
	N_C
	&=\mathcal{N}(\frac{\epsilon}{\sqrt{m}},\mbC,\rm d)
	\le \sum_{q=1}^{2\min(r,K)}\left(\frac{c \sqrt{m}(\delta+2\sqrt{\gamma})}{\epsilon}\right)^{2sq+q(\min(K^2,m)-q)} \\
	&\leq 2\min(r,K) \left(\frac{c \sqrt{m}(\delta+2\sqrt{\gamma})}{\epsilon}\right)^{2(2s+\min(K^2,m))\min(r,K)}. 
\end{align*}
For each clustering center matrix $\bC_{\epsilon,l}\in\mbC_\epsilon\subset \mbI^{2s\times \min(K^2,m)}$, one can create a set of $2s\times m$ matrices with columns randomly chosen  from $\bC_{\epsilon,l}$, i.e., 
\begin{align*}
	&\mbM_{\epsilon,l}=\{\bM_{\epsilon,l,w}\in\mbI^{2s\times m}: 
	\bM_{\epsilon,l,w} \text{  consists of columns randomly chosen  from } \\
	&\hskip 1em \bC_{\epsilon,l}, w=1,\cdots,\min(K^2,m)^m\}.
\end{align*}

By this construction, it is straightforward to see that there exists a matrix $\bM_{\epsilon,l,w}\in\mbM_{\epsilon,l}$ such that any column in $\bM_{\bB}-\bM_{\bB^*}$, say, $\bM_{\bB,j}-\bM_{\bB^*,j}$, satisfies that $\norm{\bM_{\bB,j}-\bM_{\bB^*,j}-\bM_{\epsilon,l,w,j}}_2\le \epsilon/\sqrt{m}$, where  $\bM_{\epsilon,l,w,j}$ is the $j$th column of $\bM_{\epsilon,l,w}$ for any $1\le j\le m$. Therefore, there exist a matrix $\bM_{\epsilon,l,w}\in\mbM_{\epsilon,l}$ such that ${\rm d}(\bM_{\bB}-\bM_{\bB^*},\bM_{\epsilon,l,w})\le \sqrt{m\times \epsilon^2/m}=\epsilon.$ As a result, ${\rm d}(\bM_{\bB}-\bM_{\bB^*},\bM_{\epsilon,l,w})\le \epsilon.$

In other words, $\mbM_{\epsilon}=\cup_{l=1}^{N_C} \mbM_{\epsilon,l}$ forms a $\epsilon$-covering of the space $\mbM_{rs\gamma}(\delta)$ with a carnality $\min(K^2,m)^m N_C$.

  \item[(d).] We next analyze the property of $\mbD_{rs\gamma}(\delta)$. Using inequality~\eqref{eq21} and the fact that $\rank{\bA+\bB}\le \rank{\bA}+\rank{\bB}$, it holds that
   \begin{equation}
        \label{eq2}
        \begin{aligned}
        \rank{\bB-\bM_{\bB}-(\bB^*-\bM_{\bB}^*)}&\le 2(r+\min(r,K)) \text{ and }
        \norm{\bB-\bM_{\bB}-(\bB^*-\bM_{\bB}^*)}_{2,0}&\le 2s.
        \end{aligned}
    \end{equation}

Then the following inequalities holds
  \begin{equation}
      \label{eq11}
      \begin{aligned}
		&\norm{\bB-\bM_{\bB}-(\bB^*-\bM_{\bB^*})}_F
	  \le \norm{\bB-\bM_{\bB}}_F+\norm{(\bB^*-\bM_{\bB^*})}_F\\
	  &\hskip 1em =\sqrt{P_{km}(\bB)}+\sqrt{P_{km}(\bB^*)}
	  \le 2\sqrt{\gamma}.
	  \end{aligned}
  \end{equation}
 

    
%Next, we divide the parameter space $\bDelta\mbB_{rs\gamma}(\delta)$ as $\bDelta\mbB_{rs\gamma}(\delta)=\cup_{l=1}^{C_{p}^s}\bDelta\mbB_{rs\gamma}(\delta,\mathcal{S}_l)$, where the set $\bDelta\mbB_{rs\gamma}(\delta,\mathcal{S}_l)=\{\bDelta\in\bDelta\mbB_{rs\gamma}(\delta)$ \text{ and only rows in set } $\mathcal{S}_l \text{ are non-zeros, and } |\mathcal{S}_l|=2s \}$. Note that $C_{p}^{2s}$ is the total number of ways to choose $2s$ nonzero rows out of $p$ total rows.
 %   \item[(c).] Next, we focus only on the non-zero rows of matrices in $\bDelta\mbB_{rs\gamma}(\balpha,\mathcal{S}_l)$ for a given $l$, denoted as 
 %   \[
%        \mbA_{rst}(\delta)=\{\bA:\bA\in\mbI^{s\times m}, ~ \rank{\bA} \le 2 r ~ \text{and} ~ P_{km}(\bA+\bA^*)\le t\},
%    \]
 %   where $\bA^*$ corresponds to the nonzero rows in $\bB^*$ ($s$ nonzero rows and $s$ zero rows). Note that $P_{km}(\bA)=P_{km}(\bB)$ if $\bA$ contains all non-zero rows of matrix $\bB$ by definition.
As a result, we can write $\mbD_{rs\gamma}$ as follows
    \[
    \mbD_{rs\gamma}(\delta)=\{\bD\in\mbI^{p\times m}: \norm{\bD}_F\le 2\sqrt{\gamma}, \norm{\bD}_{2,0}\le 2s, \text{ and } \rank{\bD}\le 2(r+\min(r,K))\}.
    \]
    Therefore, there exist a set of matrices $\mbD_{\epsilon}=\{\bD_{\epsilon,1},\cdots,\bD_{\epsilon,N_D}, N_D=\mathcal{N}({\epsilon},\mbD_{rs\gamma}(\delta),\rm d)\}$ such that for any $\bD\in\mbD_{rs\gamma}(\delta)$, there exist a $\bD_{\epsilon,l}\in \mbD_{\epsilon}$ such that ${\rm d}(\bD,\bD_{\epsilon,l})\le \epsilon$. Using the same arguments in the proof of Lemma 4 and Lemma 5 in~\cite{she2017selective},  we can show that 
	\begin{align*}
		N_D
		&=\mathcal{N}(\epsilon,\mbD_{rs\gamma}(\delta),{\rm d})
		\le C_p^{2s}\sum_{q=1}^{2r+2\min(r,K)}\left(\frac{c \sqrt{\gamma}}{\epsilon}\right)^{2sq+q(m-q)}\\
		&\leq 2C_p^{2s}(r+\min(r,K)) \left(\frac{c \sqrt{\gamma}}{\epsilon}\right)^{2(2s+m)(r+\min(r,K))},
	\end{align*}
	where $C_p^{2s}$ stands for choose $2s$ from $p$. 
    Therefore, for any matrix $\bDelta\in\Delta\mbB_{rs\gamma}(\delta)$, there exist a matrix $\bDelta_{l,w,l'}=\bM_{\epsilon,l,w}-\bM_{\bB^*}+\bD_{\epsilon,l'}$ from the following set 
    \[
\Delta\mbB_{\epsilon}=\mbM_{\epsilon}\oplus \mbD_{\epsilon}
    \]
    such that ${\rm d}(\bDelta,\bDelta_{l,w,l'})\le {\rm d}(\bM_{\bB}-\bM_{\bB^*},\bM_{l,w})+ {\rm d}(\bB-\bM_{\bB}-(\bB^*-\bM_{\bB^*}),\bD_{l'})\le 2\epsilon$. The cardinally 
	\begin{align*}
		|\Delta\mbB_{\epsilon}|
		&=N_C\times \min(K^2,m)^m\times N_D
		\le 2\min(r,K) \left(\frac{c \sqrt{m}(\delta+2\sqrt{\gamma})}{\epsilon}\right)^{2(2s+\min(K^2,m))\min(r,K)}
		\\
		&\quad ~ \times K^{2m}\times  2C_p^{2s}(r+\min(r,K)) \left(\frac{c \sqrt{\gamma}}{\epsilon}\right)^{2(2s+m)(r+\min(r,K))}.
	\end{align*}
 
Combining steps (a)-(d), it is straight forward to see that a $3\epsilon$-covering set $\wt\mbB_{3\epsilon}$ can be constructed by standard product spaces argument, and the cardinally of $\wt\mbB_{3\epsilon}$ is bounded as follows
\[
\begin{aligned}
 &|\wt\mbB_{3\epsilon}|\le |\mbA_{\alpha,\epsilon}| \times|\Delta\mbB_\epsilon|
 \le \underbrace{2C_{p}^{2s} \left(\frac{c\delta}{\epsilon}\right)^{mq}}_{T_1} \times 
 \underbrace{2\min(r,K) \left(\frac{c \sqrt{m}(\delta+2\sqrt{\gamma})}{\epsilon}\right)^{2(2s+\min(K^2,m))\min(r,K)}}_{T_2}\times 
 \\&\hskip10em \underbrace{K^{2m}}_{T_3} \times  \underbrace{(r+\min(r,K)) \left(\frac{c \sqrt{\gamma}}{\epsilon}\right)^{2(2s+m)(r+\min(r,K))}}_{T_4} 
\end{aligned},
\]
where it is obvious $\log T_3 = 2m \log K$. We next calculate $\log T_1, \log T_2$ and $\log T_4$, respectively. There are 
\begin{align}
	\log T_1 &= \log 2 + \log C_p^{2s} + mq \log\left(\frac{c\delta}{\epsilon}\right) \leq c_1 \left[s\log p + mq \log\left(\frac{\delta}{\epsilon}\right)\right], \label{lem:2:ineq:1}
	\\
	\log T_2 
	&= \log 2 + \log \min(r, K) + 2[2s+\min(K^2,m)]\min(r,K) \log \left(\frac{c \sqrt{m}(\delta+2\sqrt{\gamma})}{\epsilon}\right)
	\nonumber \\
	&\leq c_2 [s+\min(K^2,m)]\min(r,K) \log \left(\frac{\sqrt{m}(\delta+\sqrt{\gamma})}{\epsilon}\right),\label{lem:2:ineq:2}
\end{align}
where we use the fact the last term is dominant in $\log T_2$. As for the last $T_4$, we have 
\begin{align}
	\log T_4 
	&= \log [r+\min(r,K)] + 2(2s+m)[r+\min(r,K)]\log \left(\frac{c \sqrt{\gamma}}{\epsilon}\right)
	\nonumber \\
	&\leq c_4 (s+m)[r+\min(r,K)]\log \left(\frac{\sqrt{\gamma}}{\epsilon}\right) \leq c_4^{\prime} r(s+m) \log \left(\frac{\sqrt{\gamma}}{\epsilon}\right). \label{lem:2:ineq:3}
\end{align}
Combining \eqref{lem:2:ineq:1}--\eqref{lem:2:ineq:3}, $\log T_3$ and $\abs{\wt{\mbB}_{\epsilon}}$, we can obtain 
\begin{align*}
	&\log \mathcal{N}\left(\epsilon/2,\wt\mbB_{rs\gamma}(\delta),{\rm d}\right)
	\leq c\Bigg\{s\log p + m\log K + mq \log\left(\frac{\delta}{\epsilon}\right)
	\\
	&\quad \quad + [s+\min(K^2,m)]\min(r,K) \log \left(\frac{\sqrt{m}(\delta+\sqrt{\gamma})}{\epsilon}\right) + r(s+m) \log \left(\frac{\sqrt{\gamma}}{\epsilon}\right)\Bigg\}
\end{align*}
By basic calculus calculations, we have 
\begin{align*}
	&\int_{0}^{\delta} \sqrt{\log\left(\frac{\sqrt{m}(\delta + \sqrt{\gamma})}{\epsilon}\right)} d\epsilon= \delta \int_{0}^{1} \sqrt{\log\left(\frac{\sqrt{m}(1 + \sqrt{\gamma}/\delta)}{\epsilon}\right)} d\epsilon
	\\
	&\quad \leq \delta \int_{0}^{1} \log\left(\frac{\sqrt{m}(1 + \sqrt{\gamma}/\delta)}{\epsilon}\right) d\epsilon
	\leq c \delta \log\left(\sqrt{m}(1 + \sqrt{\gamma}/\delta)\right).
\end{align*}
When $\gamma < \delta^2$, the result of Proposition \ref{prop:2} yields $\int_{0}^{\delta} \sqrt{\log\left(\frac{\sqrt{\gamma}}{\epsilon}\right)} d\epsilon \leq \sqrt{\pi \gamma}$. Therefore, under the case $\gamma < \delta^2$, we have 
\begin{align*}
	&\int_{0}^{\delta} \sqrt{\log \mathcal{N}\left(\epsilon/2,\wt\mbB_{rs\gamma}(\delta),{\rm d}\right)} d\epsilon 
	\leq c \Bigg\{ \delta\sqrt{s\log p + m\log K} +\delta \sqrt{mq}
	\\
	&\quad + \delta\sqrt{[s+\min(K^2,m)]\min(r,K) \log m} + \sqrt{\gamma r(s+m)} \Bigg\}.
\end{align*}

% For the following simplifications, we first calculate the following two calculus 
% \begin{align*}
% 	&\int_{0}^{\delta} \sqrt{\log\left(\frac{\sqrt{m}(\delta + \sqrt{\gamma})}{\epsilon}\right)} d\epsilon
% 	= \delta \int_{0}^{1} \sqrt{\log\left(\frac{\sqrt{m}(1 + \sqrt{\gamma}/\delta)}{\epsilon}\right)} d\epsilon
% 	\\
% 	&\quad \leq \delta \int_{0}^{1} \log\left(\frac{\sqrt{m}(1 + \sqrt{\gamma}/\delta)}{\epsilon}\right) d\epsilon
% 	\leq c \delta \log\left(\sqrt{m}(1 + \sqrt{\gamma}/\delta)\right),
% 	\\
% 	&\int_{0}^{\delta} \sqrt{\log \left(\frac{\sqrt{\gamma}}{\epsilon}\right)} d \epsilon 
% 	= \delta \int_{0}^{1} \sqrt{\log \left(\frac{\sqrt{\gamma}/\delta}{\epsilon}\right)} d \epsilon \leq c \delta \text{ if } t \leq \delta^2.
% \end{align*}
% When $t \leq \delta^2$, some calculus calculations give that 
% \begin{align*}
% 	&\int_0^\delta \sqrt{\log \mathcal{N}\left(\epsilon/2,\wt\mbB_{rs\gamma}(\delta),{\rm d}\right)}d\epsilon
% 	\leq c \delta \Bigg\{\sqrt{s\log p + m \log K} + \sqrt{m} 
% 	\\
% 	&\quad \quad + \sqrt{[s+\min(K^2,m)]\min(r,K)} \log m + \sqrt{r(s+m)}
% 		\Bigg\},
% \end{align*}
% where we use the inequality $\sqrt{a + b} \leq \sqrt{a} + \sqrt{b}$.

When $\gamma > \delta^2$, we can ignore the constraint $P_{km}(\bB)\le \gamma$ in $\wt\mbB_{rs\gamma}(\delta)$,  and follow the proof of Lemma 4 and Lemma 5 in~\cite{she2017selective} to show that
\[
\begin{aligned}
    \int_0^\delta \sqrt{\log \mathcal{N}\left(\epsilon/2,\wt\mbB_{rs\gamma}(\delta),{\rm d}\right)}d\epsilon 
	\le c \delta \left(\sqrt{s\log p}+\sqrt{(s+m)r}\right),
\end{aligned}
\]
where we omit the term $\sqrt{mq}$ that is negligible compared with other terms due to the finite $q$. Using \eqref{con}, we have that
\[
\begin{aligned}
     \mbE&\left(\sup_{{\rm d}(\wt \bB,\wt \bB^*)\le\delta}\left|\wt S(\bA,\bB) - \wt S(\bA^*,\bB^*)\right|\right)\\
	 &\le 
	 c \Bigg\{ \delta\left(\sqrt{s\log p + m\log K} + \sqrt{[s+\min(K^2,m)]\min(r,K) \log m}\right)
	\\
	&\quad  + \min(\sqrt{\gamma}, \delta)\sqrt{r(s+m)} \Bigg\}
\end{aligned}
\]
for some constant $c>0$, which gives inequality~\eqref{eq:lem:3}.

\end{enumerate}
\end{proof}

\begin{proposition}\label{prop:2}
	When $z<a$, there is 
\begin{align*}
	\int_{0}^{a} \sqrt{b + c\log (z/x)} dx \leq a\sqrt{b} + z\sqrt{\pi c}.
\end{align*}
% Moreover, we have $\int_{0}^{a} \sqrt{b + c\log (z/x)} dx \leq a\sqrt{b} + z\sqrt{\pi c}$ when $z < a$. 
\end{proposition}
\begin{proof}{Proof.}
	Let $u$ be $\sqrt{b + c\log(z/x)}$ then we have 
	\begin{align*}
		\int_{0}^{a} \sqrt{b + c\log (z/x)} dx
		&= \int_{\infty}^{\sqrt{b + c\log(z/a)}} u d \left(z\exp\left(-(u^2-b)/c\right)\right)
		\\
		&= u z \exp\left(-(u^2-b)/c\right) |_{\infty}^{\sqrt{b + c\log(z/a)}} 
		\\
		&\quad - \int_{\infty}^{\sqrt{b + c\log(z/a)}} z \exp\left(-(u^2-b)/c\right) du
	\end{align*}
	By further calculations, there is 
	\begin{align*}
		\int_{0}^{a} \sqrt{b + c\log (z/x)} dx
		&= a\sqrt{b + c\log(z/a)} %\left[z \exp\left(-(b+c\log(z/a) - b) / c\right)\right]
		+ \int_{\sqrt{b + c\log(z/a)}}^{\infty} z\exp\left(-(u^2 - b) / c\right) du 
		\\
		&\leq a\sqrt{b + c \log(z/a)} + \int_{-\infty}^{\infty} z\exp\left(-(u^2 - b) / c\right) du. 
	\end{align*}
	Together with $\int_{-\infty}^{\infty} z\exp\left(-(u^2 - b) / c\right) du \leq z\sqrt{\pi c}$, we obtain 
	\begin{align*}
		\int_{0}^{a} \sqrt{b + c\log (z/x)} dx
		\leq a\sqrt{b + c \log(z/a)} + z\sqrt{\pi c} \leq a\sqrt{b} + z\sqrt{\pi c}. 
	\end{align*}
\end{proof}


==> proofs/properties.tex <==
\section{Supplementary materials}

\subsection{Basic Properties of Multinomial Logistic Model}

\noindent\textbf{1. Sub-Gaussianity}

Denote the $(m+1)$-dimensional random vector by $\y = (y_1,\dots, y_m,y_{m+1})\in\mbR^{m+1}$, whose distribution is 
\begin{align*}
	\mbP(y_i = 1) = p_i^*, ~ \mbP(y_i = 0) = 1 - p_i^*,
\end{align*}
with $\sum_{i=1}^{m+1} p_i^* = 1$ and $i=1,\dots,m,m+1$. Let $\a\in\mbR^{m+1}$ be an arbitrary deterministic vector with $\norm{\a}_2=1$ then we consider the upper bound of $\mbE \left\{\exp[\a\trans(\y - \p^*)]^2\right\}$. Note that the distribution of $\a\trans \y$ follows $\bP(\a\trans \y = a_i) = p_i^* , \, i= 1,\dots, m, m+1$. Then we have 
\begin{align*}
	\mbE \left\{\exp[\a\trans(\y - \p^*)]^2\right\}
	&= \sum_{i=1}^{m+1} p_i^* \exp\left[a_i^2 + (\a\trans\p^*)^2 - 2a_i\a\trans\p^*\right]
	\\
	&\leq \exp\left[(\a\trans\p^*)^2 \right] \left[\max_{i}\, \exp (a_i^2)\sum_{i=1}^{m+1} p_i^*\right] 
	\triangleq 2C^2 < + \infty,
\end{align*}
where $C$ is an absolute positive constant. Applying Markov's inequality, we can obtain 
\begin{align*}
	\mbP \left(\abs{\a\trans(\y - \p^*)} > t\right) 
	&= \mbP \left\{\exp\left[\frac{\a\trans(\y - \p^*)}{C}\right]^2 > \exp \left(\frac{t^2}{C^2}\right)\right\} 
	\leq \frac{\mbE \exp\left[\a\trans(\y - \p^*)/C\right]^2}{\exp \left(t^2/C^2\right)}
	\\
	&\leq 2\exp \left(-\frac{t^2}{C^2}\right),
\end{align*}
which proves the sub-Gaussianity of $\y$. 

\noindent\textbf{2. Derivative}

Let $\ell(\bB)$ be the negative log-likelihood of the multinomial logistic model that is 
\begin{align*}
	\ell(\bB) 
	&= \sum_{i=1}^n b(\bB\trans\x_i) - \trace{\bY\trans\bX\bB}
	\\
	&= \sum_{i=1}^n \log\left[1 + \sum_{j=1}^m \exp(\x_i\trans\bbeta_j)\right] - \sum_{i=1}^n \sum_{j=1}^m y_{ij}\bbeta_j\trans\x_i,
\end{align*}
where $\bbeta_j\in \mbR^p$ is the $j$-th column of $\bB$ and we put the intercept into the covariate $\x_i$ for convenience. Then we have the first derivative of $\ell(\bB)$ as follows 
\begin{align*}
	\nabla \ell(\bbeta_l) 
	= \sum_{i=1}^n \frac{\exp(\x_i\trans\bbeta_l)\x_i}{1 + \sum_{j=1}^m \exp(\x_i\trans\bbeta_j)} - \sum_{i=1}^n y_{il}\x_i,
\end{align*}
where $\nabla \ell(\bbeta_l)$ is the $l$-th column of $\nabla \ell(\bB)$. It ensures $\mbE [\nabla \ell(\bB^*)] = \0_{n\times m}$. Let $\nabla^2 \ell(\bbeta_{l,k}) \in \mbR^{p\times p}$ be the derivative of $\nabla \ell(\bbeta_l)$ in term of $\bbeta_k\trans$. Then we can obtain that 
\begin{equation*}
	\nabla^2 \ell(\bbeta_{l,k}) = \left\{
	\begin{aligned}
		&-\sum_{i=1}^n \frac{\exp[\x_i\trans(\bbeta_l + \bbeta_k)]}{[1 + \sum_{j=1}^m \exp(\x_i\trans\bbeta_j)]^2}\x_i\x_i\trans, \quad l \neq k
		\\
		& \sum_{i=1}^n \frac{\exp(\x_i\trans\bbeta_l)[1-\exp(\x_i\trans\bbeta_l)]}{[1 + \sum_{j=1}^m \exp(\x_i\trans\bbeta_j)]^2} \x_i\x_i\trans, \quad l =k
	\end{aligned}
	\right..
\end{equation*}
Therefore, the Hessian $\nabla^2\ell(\bB)$ is a $mp\times mp$ matrix that is composed by the blocks $\nabla^2 \ell(\bbeta_{l,k})$ with $l,k=1,\dots,m$. Let $\p_i^*$ be the expectation of the $i$-th response $y_i$. Following $\p_i^*$, we define the matrix $\bH_i^* = \diag{\p_i^*} - \p_i^*\p_i\strans \in \mbR^{m\times m}$. Then the Hessian matrix $\nabla^2 \ell(\bB^*)$ can be reformulated as $\nabla^2 \ell(\bB^*) = \sum_{i=1}^n \bH_i^* \otimes \x_i\x_i\trans$, where $\otimes$ is Kronecker product. Finally, it is obvious that $\nabla^2 \ell(\bB) = \nabla^2 b(\bB)$ since another term in $\ell(\bB)$ is linear. 




==> proofs/theorems.tex <==
% Recall that the negative log-likelihood $\ell(\bA,\bB)$ and its derivative as follows
% \begin{align*}
% 	&\ell(\bA,\bB) = \sum_{i=1}^n b(\bA\trans\z_i+\bB\trans\x_i) - \trace{\bY\trans(\bZ\bA+\bX\bB)}, \\
% 	&\nabla \ell(\bA,\bB)
% 	= \sum_{i=1}^n \wt\x_i \der{b}{\btheta_i\trans} - \wt\bX\trans\bY
% 	= \sum_{i=1}^n \wt\x_i \left(\der{b}{\btheta_i\trans} - \y_i\trans\right)
% \end{align*}
% % Then the partial derivative of $\ell(\bA,\bB)$ is of the form
% % \begin{align*}
% % 	\nabla \ell(\bA,\bB)
% % 	= \sum_{i=1}^n \wt\x_i \der{b}{\btheta_i\trans} - \wt\bX\trans\bY
% % 	= \sum_{i=1}^n \wt\x_i \left(\der{b}{\btheta_i\trans} - \y_i\trans\right),
% % \end{align*}
% where $\btheta_i = \bA\trans\z_i+\bB\trans\x_i$, $\wt \x_i=(\z_i\trans,\x_i\trans)\trans\in\mbR^{q+p}$, $\wt\bX = [\wt\x_1,\dots,\wt\x_n]\trans$ and $\bY = [\y_1,\dots,\y_n]\trans$. We will use these two notations later.

% \section{Proofs of Main Results}

\section{Proofs of Theorem \ref{thm:1}}

Denote by $\wt\bB=[\bA\trans,\bB\trans]\trans$ and $\wh{\wt\bB}=[\wh\bA\trans;\wh\bB\trans]\trans$. Correspondingly, the true coefficient matrix is $\wt{\bB}^* = [\bA\strans,\bB\strans]\trans$ and recall the parameter space
\begin{equation}
	\label{psp-2}
	\begin{aligned}
		\wt\mbB_{rs\gamma}=\{\wt\bB=[\bA\trans,\bB\trans]\trans:\bA\in\mbR^{q\times m},\bB\in\mbR^{p\times m},\norm{\bB}_{2,0} \leq s, ~ \rank{\bB} \leq r,~ \text{and} ~ P_{km}(\bB)\le \gamma\},
	\end{aligned}
\end{equation}
which satisfies that $\wt{\bB}^* \in \wt\mbB_{rs\gamma}$. For a given $L_n > 0$, we partition the parameter space as
\[
	\wt\mbB_{rs\gamma}=\cup_{j=1}^{\infty} \wt\mbB_{rs\gamma,j},~\text{ where }\wt\mbB_{rs\gamma,j}=\{ \wt\bB\in\wt\mbB_{rs\gamma}: 2^{j-1}\le L_n{\rm d} (\wt\bB,\wt\bB^*)<2^j\}.
\]
If $L_n{\rm d} (\wh{\wt\bB},\wt\bB^*)>2^Q$ for some integer $Q$, we have $\wh{\wt\bB}\in \wt\mbB_{rs\gamma,j}$ for some $j>Q$. Then by the definition of $\wh{\wt\bB}$, we have that $\ell(\wh{\wt\bB})\le \ell(\wt\bB^*) $, and hence
\[
	\begin{aligned}
		\mbP\left(L_n{\rm d} (\wh{\wt\bB},\wt\bB^*)>2^Q \right)&= \mbP\left(\wh{\wt\bB}\in\cup_{j=Q}^{\infty} \wt\mbB_{rs\gamma,j} \right)\le \mbP\left(\inf_{\wt\bB\in\cup_{j=Q}^{\infty} \wt\mbB_{rs\gamma,j}}\left[\ell(\wt\bB)- \ell(\wt\bB^*)\right]\le 0 \right)\\
		&\le \sum_{j=Q}^{\infty}\mbP\left(\inf_{\wt\bB\in \wt\mbB_{rs\gamma,j}}\left[\ell(\wt\bB)- \ell(\wt\bB^*)\right]\le 0 \right)\\
		&\le \sum_{j=Q}^{\infty}\mbP\left(\inf_{\wt\bB\in \wt\mbB_{rs\gamma,j}}\left[S(\wt\bB)- S(\wt\bB^*)+\mbE\left(\ell(\wt\bB)-\ell(\wt\bB^*)\right)\right]\le 0 \right)\\
		&\le \sum_{j=Q}^{\infty}\mbP\left(\inf_{\wt\bB\in \wt\mbB_{rs\gamma,j}}\left[S(\wt\bB)- S(\wt\bB^*)\right]+\inf_{\wt\bB\in \wt\mbB_{rs\gamma,j}}\mbE\left[\ell(\wt\bB)-\ell(\wt\bB^*)\right]\le 0 \right),
	\end{aligned}
\]
where $S(\wt\bB)=\ell(\wt\bB)-\mbE\left[\ell(\wt\bB)\right]=\ell(\bA,\bB)-\mbE\left[\ell(\bA,\bB)\right]$. Note that
\[
	\begin{aligned}
		\mbE\left[\ell(\wt\bB)-\ell(\wt\bB^*)\right]
		&=b(\wt\bB)-b(\wt\bB^*)-\trace{\mbE{\bY}\trans \wt\bX(\wt\bB-\wt\bB^*)}\\
		&=b(\wt\bB)-b(\wt\bB^*)-\trace{\nabla b(\wt\bB^*)\trans(\wt\bB-\wt\bB^*)}\\
		&=b(\wt\bB)-b(\wt\bB^*)-\inner{\nabla b(\wt\bB^*),\wt\bB-\wt\bB^*}
		\ge \frac{n\kappa}{2}\norm{\wt\bB-\wt\bB^*}_F^2,
	\end{aligned}
\]
where the last inequality follows from Condition~\ref{cond:1}. Then for any $\wt\bB\in \wt\mbB_{rs\gamma,j}$, it holds that
\[
	\mbE\left[\ell(\wt\bB)-\ell(\wt\bB^*)\right]\ge L_n^{-2}n\kappa 2^{2j-3},
\]
which implies that
\[
	\begin{aligned}
		\mbP\left(L_n{\rm d} (\wh{\wt\bB},\wt\bB^*)>2^Q \right)&\le \sum_{j=Q}^{\infty}\mbP\left(\inf_{\wt\bB\in \wt\mbB_{rs\gamma,j}}\left[S(\wt\bB)- S(\wt\bB^*)\right]+L_n^{-2}n\kappa 2^{2j-3}\le 0 \right)\\
		&\le \sum_{j=Q}^{\infty}\mbP\left(\inf_{{\rm d} (\wt\bB,\wt\bB^*)<L_n^{-1}2^j}\left[S(\wt\bB)- S(\wt\bB^*)\right]+L_n^{-2}n\kappa 2^{2j-3}\le 0 \right)\\
		&\le \sum_{j=Q}^{\infty}\mbP\left(\sup_{{\rm d} (\wt\bB,\wt\bB^*)<L_n^{-1}2^j}\left|S(\wt\bB)- S(\wt\bB^*)\right|\ge L_n^{-2}n\kappa 2^{2j-3} \right).
	\end{aligned}
\]
Furthermore by the Markov inequality, it holds that $P(|X|>x)\le \frac{E|X|}{x}$, we have that
\begin{align*}
	 \mbP\left(L_n{\rm d} (\wh{\wt\bB},\wt\bB^*)>2^Q \right)
	& \le \sum_{j=Q}^{\infty}\frac{L_n^2}{n\kappa 2^{2j-3}} \mbE\left(\sup_{{\rm d} (\wt\bB,\wt\bB^*)<L_n^{-1}2^j}\left|S(\wt\bB)- S(\wt\bB^*)\right| \right) \\
	& \lesssim \sum_{j=Q}^{\infty}\frac{L_n^2\times L_n^{-1}2^j}{n\kappa 2^{2j-3}} \norm{\wt \bX}_{2s,op}
	\Bigg[
	\min\left(\frac{\sqrt{\gamma}}{L_n^{-1}2^j},1\right)\times                                                  \\
	 & \hskip 3em \sqrt{(s+m)r} + \sqrt{s\log p+m\log K}+\sqrt{[s+\min(K^2,m)]\min(r,K)\log m}
		\Bigg],
\end{align*}
for some constant, where we use Lemma \ref{lem:3} (in the supplementary material) in the last inequality. By further simplifications, we can obtain
\begin{align*}
	 & \mbP\left(L_n{\rm d} (\wh{\wt\bB},\wt\bB^*)>2^Q \right)
	\lesssim \frac{L_n\norm{\wt{\bX}}_{2s,\op}\sqrt{(s+m)r}}{n\kappa} \sum_{j=Q}^{\infty} \frac{\min\left(\frac{\sqrt{\gamma}}{L_n^{-1}2^j},1\right)}{2^{j-3}}
	\\
	 & \hskip 2em + \frac{L_n\norm{\wt{\bX}}_{2s,\op}\left(\sqrt{s\log p+m\log K}+\sqrt{[s+\min(K^2,m)]\min(r,K)\log m}\right)}{n\kappa} \sum_{j=Q}^{\infty} \frac{1}{2^{j-3}}.
\end{align*}

	\noindent (a). {\bf Case I: if $L_n\sqrt{\gamma}=O(1)$.} Then for a sufficiently large $Q$, it holds that
	      \[
		      \begin{aligned}
			      &\mbP\left(L_n{\rm d} (\wh{\wt\bB},\wt\bB^*)>2^Q \right)
			      \lesssim \Big[\sqrt{\gamma} \sqrt{(s+m)r} + \sqrt{s\log p+m\log K} \\
				  &\hspace{3em} + \sqrt{[s+\min(K^2,m)]\min(r,K)\log m}\Big]\frac{L_n\norm{\wt \bX}_{2s,op}}{2^{Q-3}n\kappa}.
		      \end{aligned}
	      \]
	      We take that
	      \begin{align*}
		      L_n^{-1}
		       = \Big[\sqrt{r\gamma(s+m)} + \sqrt{s\log p+m\log K}
		      + \sqrt{[s+\min(K^2,m)]\min(r,K)\log m}\Big]\frac{\norm{\wt \bX}_{2s,op}}{n\kappa}
	      \end{align*}
	      Then, if
	      \begin{align*}
		      \frac{n^2\kappa^2 \gamma}{\min \{s\log p+m\log K,\, [s+\min(K^2,m)]\min(r,K)\log(m),\, r(s+m)\} \norm{\wt \bX}_{2s,op}^2} = O(1),
	      \end{align*}
	      it holds that $L_n\sqrt{\gamma}=O(1)$.

	\noindent (b). {\bf Case II: if $L_n\sqrt{\gamma}\to\infty$.}
	      In this case, we have that
	      \[
		      \begin{aligned}
			      \mbP\left(L_n{\rm d} (\wh{\wt\bB},\wt\bB^*)>2^Q \right)
			      &\lesssim
			      \frac{1}{2^{Q-3}} \frac{L_n \norm{\wt \bX}_{2s,op}}{n\kappa} \Bigg(\sqrt{(s+m)r} + \sqrt{s\log p+m\log K}
			      \\
			      &\hskip 2em + \sqrt{[s+\min(K^2,m)]\min(r,K)\log m}\Bigg).
		      \end{aligned}
	      \]
	      In this case, we can take
	      \begin{align*}
		      L_n^{-1}
		      = \frac{\norm{\wt \bX}_{2s,op}}{n\kappa} \Bigg(\sqrt{(s+m)r} + \sqrt{s\log p+m\log K}
		      + \sqrt{[s+\min(K^2,m)]\min(r,K)\log m}\Bigg).
	      \end{align*}
	      and then if
	      \begin{align*}
		      \frac{n^2\kappa^2 \gamma}{\min \{s\log p+m\log K,\, [s+\min(K^2,m)]\min(r,K)\log(m),\, r(s+m)\} \norm{\wt \bX}_{2s,op}^2} \rightarrow +\infty,
	      \end{align*}
	      it holds that $L_n\sqrt{\gamma}\rightarrow + \infty$.

Therefore, the convergence rate of ${\rm d} (\wh{\wt\bB},\wt\bB^*)$ is of the order $O_p(L_n^{-1})$, which gives the convergence rates as follows
\begin{enumerate}
	\item[(a).] If  $\frac{\kappa^2 \gamma}{\zeta_n^2}=O(1)$ as $n\to\infty$, we have
	\begin{align*}
		   \norm{\wh\bA-\bA^*}_F+\norm{\wh\bB-\bB^*}_F = O_P\left(
			   \frac{\xi_{m,K}(\gamma)\norm{\wt \bX}_{2s,op}}{n\kappa}
			   \right);
	\end{align*}
	\item[(b).] If $\frac{\kappa^2 \gamma}{\zeta_n^2}\to\infty$ as $n\to\infty$, we have
	\begin{align*}
	   \norm{\wh\bA-\bA^*}_F+\norm{\wh\bB-\bB^*}_F = O_P\left(
	   \frac{\xi_{m,K}(1)\norm{\wt \bX}_{2s,op}}{n\kappa}
	   \right).
	\end{align*}
\end{enumerate}
Finally, we apply Condition \ref{cond:2} that concludes the parts (a) and (b) of Theorem \ref{thm:1}.



==> table.tex <==
\begin{tabular}{ccccccccccc} 
    \toprule 
    $\epsilon$ & Method & Er$(\bB)$ & KL$\times 10$ & Time (s) & Er$(\bB)$ & KL$\times 10$ & Time (s) & Er$(\bB)$ & KL$\times 10$ & Time (s)
     \\ \hline 
     &&\multicolumn{3}{c}{$n_{ratio}=50$} & \multicolumn{3}{c}{$n_{ratio}=100$} & \multicolumn{3}{c}{$n_{ratio}=200$}
     \\ 
    \hline 
    \multirow{2}{*}{$0.9$} & SRRR &  14.3 &  0.48 &  9.28 &  6.9 &  0.29 &  11.97 &  3.31 &  0.13 &  22.55
     \\ 
      & Laplacian-penalty &  11.38 &  0.44 &  36.98 &  6.32 &  0.26 &  71.97 &  3.91 &  0.13 &  170.11
     \\ 
     \hline 
    \multirow{2}{*}{$0.6$} & SRRR &  14.53 &  0.49 &  9.51 &  6.3 &  0.25 &  10.66 &  3.82 &  0.15 &  19.68
     \\ 
      & Laplacian-penalty &  10.72 &  0.43 &  35.04 &  6.08 &  0.23 &  52.71 &  3.78 &  0.13 &  115.89
     \\ 
     \hline 
    \multirow{2}{*}{$0.3$} & SRRR &  13.35 &  0.46 &  8.81 &  7.53 &  0.24 &  10.92 &  3.57 &  0.12 &  20.92
     \\ 
      & Laplacian-penalty &  9.96 &  0.34 &  29.35 &  7.83 &  0.21 &  41.57 &  3.19 &  0.09 &  91.52
     \\ 
     \bottomrule 
     \end{tabular}

==> tables/2024-09-12/linear/nonsparse/rank-3-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  19.29 &  10.32 &  10.05 &  9.34 &  8.57 &  10.59
 \\ 
  & SRRR &  7.06 &  4.87 &  4.02 &  4.51 &  3.38 &  5.06
 \\ 
  & Laplacian &  7.01 &  4.87 &  4.06 &  4.53 &  3.38 &  5.05
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  15.63 &  8.36 &  9 &  8.36 &  7.74 &  9.56
 \\ 
  & SRRR &  6.05 &  4.12 &  3.65 &  4.08 &  3.14 &  4.67
 \\ 
  & Laplacian &  5.52 &  3.91 &  3.5 &  3.96 &  3 &  4.54
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  15.61 &  8.35 &  8.86 &  8.23 &  7.67 &  9.48
 \\ 
  & SRRR &  4.32 &  3.4 &  3.01 &  3.58 &  2.58 &  4.13
 \\ 
  & Laplacian &  3.65 &  2.86 &  2.64 &  3.15 &  2.33 &  3.76
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/linear/nonsparse/rank-6-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  25.42 &  13.52 &  12.84 &  12.05 &  9.68 &  12.09
 \\ 
  & SRRR &  15.57 &  10.05 &  8.32 &  8.91 &  6.37 &  8.91
 \\ 
  & Laplacian &  15.17 &  9.91 &  8.2 &  8.83 &  6.29 &  8.83
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  19.46 &  10.35 &  10.61 &  9.96 &  7.7 &  9.62
 \\ 
  & SRRR &  12.94 &  8.2 &  7.5 &  7.84 &  5.4 &  7.39
 \\ 
  & Laplacian &  10.25 &  6.96 &  6.29 &  6.89 &  4.68 &  6.69
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  19.53 &  10.38 &  10.75 &  10.09 &  7.79 &  9.73
 \\ 
  & SRRR &  6.4 &  5.11 &  4.87 &  5.8 &  3.96 &  6.16
 \\ 
  & Laplacian &  5.19 &  4.24 &  3.93 &  4.93 &  3.2 &  5.32
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/linear/nonsparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  13.32 &  7.06 &  8.1 &  7.5 &  5.53 &  6.84
 \\ 
  & SRRR &  7.63 &  5.02 &  4.79 &  5.31 &  3.25 &  4.84
 \\ 
  & Laplacian &  7.12 &  4.81 &  4.57 &  5.17 &  3.08 &  4.69
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  12.35 &  6.54 &  7.45 &  6.89 &  5.11 &  6.32
 \\ 
  & SRRR &  5.87 &  4.33 &  4.36 &  4.91 &  3.08 &  4.56
 \\ 
  & Laplacian &  4.7 &  3.62 &  3.56 &  4.18 &  2.52 &  3.92
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  12.21 &  6.47 &  7.38 &  6.83 &  5.06 &  6.25
 \\ 
  & SRRR &  3.3 &  2.82 &  2.41 &  3.24 &  1.79 &  3.34
 \\ 
  & Laplacian &  2.35 &  2.13 &  1.76 &  2.52 &  1.36 &  2.66
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/linear/sparse/rank-3-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  42.14 &  22.64 &  22.85 &  17.55 &  13.98 &  16.44
 \\ 
  & SRRR &  8.9 &  7.25 &  4.62 &  5.23 &  3.17 &  4.95
 \\ 
  & Laplacian &  8.83 &  7.22 &  4.55 &  5.18 &  3.16 &  4.93
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  21.7 &  15.21 &  14.5 &  13.99 &  10.36 &  13.29
 \\ 
  & SRRR &  8.54 &  6.69 &  4.94 &  5.43 &  2.95 &  4.57
 \\ 
  & Laplacian &  9.16 &  6.64 &  4.65 &  5.2 &  2.81 &  4.42
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  21.76 &  15 &  14.55 &  13.87 &  10.51 &  13.18
 \\ 
  & SRRR &  6.37 &  5.47 &  3.67 &  4.56 &  2.62 &  4.23
 \\ 
  & Laplacian &  7.02 &  4.92 &  3.15 &  3.94 &  2.32 &  3.78
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/linear/sparse/rank-6-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  39.27 &  19.31 &  21.18 &  20.22 &  15.15 &  19.09
 \\ 
  & SRRR &  13.42 &  8.92 &  8.63 &  9.38 &  5.67 &  8.34
 \\ 
  & Laplacian &  13.97 &  9.28 &  8.39 &  9.16 &  5.53 &  8.21
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  33.17 &  16.65 &  18.56 &  17.44 &  11.7 &  14.62
 \\ 
  & SRRR &  13.5 &  8.79 &  8.15 &  8.6 &  4.79 &  6.87
 \\ 
  & Laplacian &  14.39 &  9.52 &  10.19 &  10.03 &  4.29 &  6.38
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  31.03 &  15.99 &  17.85 &  16.96 &  11.4 &  14.3
 \\ 
  & SRRR &  7.71 &  5.76 &  4.94 &  6.61 &  3.68 &  6.32
 \\ 
  & Laplacian &  9.37 &  6.37 &  6.02 &  7 &  2.92 &  5.33
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/linear/sparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  20.47 &  11.46 &  15.48 &  11.63 &  8.5 &  10.31
 \\ 
  & SRRR &  6.69 &  5.06 &  4.33 &  4.73 &  2.7 &  4.15
 \\ 
  & Laplacian &  6.34 &  4.85 &  4.09 &  4.58 &  2.64 &  4.08
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  17.74 &  10.24 &  15.45 &  11.12 &  7.73 &  9.39
 \\ 
  & SRRR &  5.4 &  4.39 &  3.97 &  4.48 &  2.67 &  3.98
 \\ 
  & Laplacian &  5.49 &  4.18 &  3.48 &  4.01 &  2.11 &  3.39
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  17.57 &  10.13 &  15.37 &  11.02 &  7.6 &  9.25
 \\ 
  & SRRR &  3.07 &  2.94 &  2.06 &  3.07 &  1.57 &  2.99
 \\ 
  & Laplacian &  4.74 &  3.21 &  1.93 &  2.63 &  1.19 &  2.38
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/multi-logit/nonsparse/rank-3-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  5.11 &  11.24 &  5.32 &  12.47 &  5.21 &  11.96
 \\ 
  & SRRR &  3.49 &  3.03 &  2.22 &  2.05 &  1.87 &  1.61
 \\ 
  & Laplacian &  3.16 &  2.77 &  2.14 &  1.95 &  1.99 &  1.54
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  4.32 &  10.27 &  4.32 &  10.17 &  4.32 &  9.93
 \\ 
  & SRRR &  2.99 &  2.58 &  2.02 &  1.74 &  1.51 &  1.32
 \\ 
  & Laplacian &  2.7 &  2 &  1.91 &  1.31 &  1.44 &  1.01
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  4.27 &  10.2 &  4.26 &  10.09 &  4.27 &  9.86
 \\ 
  & SRRR &  2.91 &  2.46 &  1.91 &  1.64 &  1.41 &  1.24
 \\ 
  & Laplacian &  2.59 &  1.7 &  1.69 &  1.02 &  1.22 &  0.73
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/multi-logit/nonsparse/rank-6-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  5.75 &  12.52 &  5.28 &  11.69 &  5.55 &  11.58
 \\ 
  & SRRR &  4.19 &  3.77 &  2.83 &  2.76 &  2.53 &  2.26
 \\ 
  & Laplacian &  3.57 &  3.3 &  2.61 &  2.45 &  2.4 &  1.97
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  4.36 &  10.62 &  4.35 &  10.43 &  4.36 &  10.01
 \\ 
  & SRRR &  2.89 &  2.65 &  1.95 &  1.79 &  1.57 &  1.41
 \\ 
  & Laplacian &  2.53 &  1.98 &  1.79 &  1.29 &  1.48 &  1.01
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  4.25 &  10.42 &  4.24 &  10.21 &  4.25 &  9.79
 \\ 
  & SRRR &  2.96 &  2.51 &  1.91 &  1.65 &  1.48 &  1.24
 \\ 
  & Laplacian &  2.56 &  1.69 &  1.65 &  1.02 &  1.28 &  0.72
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/multi-logit/nonsparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  4.35 &  3.69 &  4.41 &  3.51 &  4.36 &  3.73
 \\ 
  & SRRR &  3.93 &  2.44 &  2.88 &  1.72 &  2.3 &  1.33
 \\ 
  & Laplacian &  3.95 &  2.15 &  3.02 &  1.54 &  2.43 &  1.19
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  4.04 &  3.43 &  4.03 &  3.21 &  4.03 &  3.34
 \\ 
  & SRRR &  3.62 &  2.24 &  2.62 &  1.52 &  1.98 &  1.13
 \\ 
  & Laplacian &  3.52 &  1.88 &  2.75 &  1.31 &  2.09 &  0.98
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  4 &  3.4 &  3.99 &  3.18 &  3.99 &  3.31
 \\ 
  & SRRR &  3.66 &  2.23 &  2.56 &  1.51 &  1.93 &  1.12
 \\ 
  & Laplacian &  3.56 &  1.91 &  2.66 &  1.29 &  2.03 &  0.95
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/multi-logit/sparse/rank-3-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  5.34 &  11.84 &  5.41 &  12.09 &  5.74 &  11.89
 \\ 
  & SRRR &  4.75 &  3.89 &  3.05 &  2.38 &  2.43 &  1.91
 \\ 
  & Laplacian &  3.27 &  3.03 &  2.46 &  2.07 &  2.2 &  1.78
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  4.42 &  10.22 &  4.4 &  9.9 &  4.39 &  10.1
 \\ 
  & SRRR &  4.49 &  3.63 &  2.87 &  2.35 &  2.13 &  1.76
 \\ 
  & Laplacian &  2.82 &  2.36 &  1.95 &  1.45 &  1.5 &  1.08
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  4.36 &  10.15 &  4.35 &  9.83 &  4.34 &  10.03
 \\ 
  & SRRR &  4.33 &  3.51 &  2.84 &  2.26 &  2.04 &  1.65
 \\ 
  & Laplacian &  2.81 &  2.14 &  1.81 &  1.19 &  1.34 &  0.82
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/multi-logit/sparse/rank-6-K-3.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  6.44 &  12.78 &  5.79 &  11.97 &  5.57 &  12.66
 \\ 
  & SRRR &  5.99 &  5.44 &  3.74 &  3.45 &  3.13 &  2.78
 \\ 
  & Laplacian &  4.3 &  4.51 &  2.9 &  2.96 &  2.48 &  2.37
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  4.47 &  10.03 &  4.45 &  10.02 &  4.44 &  10.16
 \\ 
  & SRRR &  4.51 &  3.72 &  2.83 &  2.46 &  2.25 &  1.88
 \\ 
  & Laplacian &  2.96 &  2.59 &  2.02 &  1.67 &  1.71 &  1.31
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  4.35 &  9.8 &  4.33 &  9.81 &  4.33 &  9.94
 \\ 
  & SRRR &  4.23 &  3.44 &  2.86 &  2.35 &  2.17 &  1.7
 \\ 
  & Laplacian &  2.7 &  2.19 &  1.98 &  1.44 &  1.59 &  1.03
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-12/multi-logit/sparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  4.39 &  3.86 &  4.42 &  3.76 &  4.41 &  3.65
 \\ 
  & SRRR &  6.44 &  3.16 &  4.18 &  2.13 &  3.23 &  1.66
 \\ 
  & Laplacian &  4.05 &  2.31 &  3.11 &  1.68 &  2.58 &  1.35
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  4.11 &  3.46 &  4.11 &  3.44 &  4.1 &  3.38
 \\ 
  & SRRR &  6.21 &  2.92 &  4.07 &  1.96 &  2.91 &  1.43
 \\ 
  & Laplacian &  3.86 &  2.08 &  2.95 &  1.49 &  2.26 &  1.12
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  4.08 &  3.43 &  4.07 &  3.41 &  4.06 &  3.35
 \\ 
  & SRRR &  6.16 &  2.91 &  3.99 &  1.87 &  2.98 &  1.39
 \\ 
  & Laplacian &  3.77 &  2.04 &  2.93 &  1.44 &  2.3 &  1.08
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-15/linear/nonsparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  12.57 &  6.66 &  7.64 &  7.07 &  5.24 &  6.47
 \\ 
  & SRRR &  7.25 &  4.76 &  4.55 &  5.03 &  3.08 &  4.59
 \\ 
  & Laplacian &  6.63 &  4.5 &  4.23 &  4.8 &  2.92 &  4.45
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  11.96 &  6.33 &  7.25 &  6.71 &  4.95 &  6.12
 \\ 
  & SRRR &  4.9 &  4.02 &  3.84 &  4.55 &  2.91 &  4.44
 \\ 
  & Laplacian &  4.04 &  3.43 &  3.11 &  3.81 &  2.33 &  3.74
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  11.87 &  6.29 &  7.2 &  6.66 &  4.91 &  6.07
 \\ 
  & SRRR &  3.38 &  2.79 &  2.3 &  3.05 &  1.61 &  2.9
 \\ 
  & Laplacian &  1.9 &  1.91 &  1.42 &  2.16 &  1.06 &  2.14
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-15/linear/sparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction  & Er$(\bB) \times 10^2$ & Prediction 
 \\ \hline 
 &&\multicolumn{2}{c}{$n=100$} & \multicolumn{2}{c}{$n=150$} & \multicolumn{2}{c}{$n=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  19.63 &  10.7 &  16.5 &  11.47 &  8.36 &  9.95
 \\ 
  & SRRR &  6.3 &  4.73 &  4.2 &  4.57 &  2.64 &  4.04
 \\ 
  & Laplacian &  5.79 &  4.44 &  3.85 &  4.35 &  2.53 &  3.94
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  18.43 &  9.89 &  15.23 &  10.67 &  7.3 &  8.86
 \\ 
  & SRRR &  5 &  4.39 &  3.65 &  4.35 &  2.57 &  3.89
 \\ 
  & Laplacian &  4.06 &  3.75 &  2.9 &  3.7 &  2.17 &  3.42
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  18.12 &  9.72 &  15.08 &  10.53 &  7 &  8.62
 \\ 
  & SRRR &  3.59 &  3.01 &  2.3 &  3 &  1.49 &  2.71
 \\ 
  & Laplacian &  2.39 &  2.14 &  1.34 &  2.03 &  0.96 &  1.91
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-15/multi-logit/nonsparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  4.16 &  4.08 &  4.2 &  3.92 &  4.15 &  3.85
 \\ 
  & SRRR &  3.75 &  2.41 &  2.55 &  1.66 &  1.83 &  1.25
 \\ 
  & Laplacian &  3.47 &  2 &  2.58 &  1.43 &  1.93 &  1.09
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  3.94 &  3.78 &  3.94 &  3.54 &  3.94 &  3.69
 \\ 
  & SRRR &  3.47 &  2.25 &  2.34 &  1.52 &  1.7 &  1.13
 \\ 
  & Laplacian &  3.17 &  1.82 &  2.37 &  1.28 &  1.83 &  0.95
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  3.91 &  3.75 &  3.91 &  3.51 &  3.91 &  3.66
 \\ 
  & SRRR &  3.49 &  2.26 &  2.28 &  1.48 &  1.71 &  1.11
 \\ 
  & Laplacian &  3.21 &  1.83 &  2.28 &  1.24 &  1.82 &  0.93
 \\ 
 \bottomrule 
 \end{tabular}

==> tables/2024-09-15/multi-logit/sparse/rank-6-K-6.tex <==
\begin{tabular}{cccc||cc||cc} 
\toprule 
$\epsilon$ & Method & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$ & Er$(\bB)$ & KL $\times 10^2$
 \\ \hline 
 &&\multicolumn{2}{c}{$n_{ratio}=100$} & \multicolumn{2}{c}{$n_{ratio}=150$} & \multicolumn{2}{c}{$n_{ratio}=200$}
 \\ 
\hline 
\multirow{3}{*}{$1.8$} & gLasso &  4.25 &  3.96 &  4.24 &  3.98 &  4.23 &  3.96
 \\ 
  & SRRR &  6.12 &  3.11 &  4.04 &  2.07 &  2.98 &  1.58
 \\ 
  & Laplacian &  3.62 &  2.19 &  2.69 &  1.57 &  2.12 &  1.25
 \\ 
 \hline 
\multirow{3}{*}{$0.6$} & gLasso &  4.03 &  3.81 &  4.02 &  3.78 &  4.01 &  3.72
 \\ 
  & SRRR &  6.07 &  2.93 &  3.83 &  1.92 &  2.83 &  1.41
 \\ 
  & Laplacian &  3.41 &  1.94 &  2.44 &  1.41 &  1.9 &  1.08
 \\ 
 \hline 
\multirow{3}{*}{$0.2$} & gLasso &  4 &  3.78 &  3.99 &  3.76 &  3.99 &  3.69
 \\ 
  & SRRR &  5.91 &  2.9 &  3.88 &  1.87 &  2.89 &  1.41
 \\ 
  & Laplacian &  3.26 &  1.92 &  2.45 &  1.35 &  2 &  1.06
 \\ 
 \bottomrule 
 \end{tabular}
